Multi-Factor Spatio-Temporal Prediction based on Graph Decomposition Learning

Spatio-temporal (ST) prediction is an important and widely used technique in data mining and analytics, especially for ST data in urban systems such as transportation data. In practice, the ST data generation is usually influenced by various latent factors tied to natural phenomena or human socioeconomic activities, impacting specific spatial areas selectively. However, existing ST prediction methods usually do not refine the impacts of different factors, but directly model the entangled impacts of multiple factors. This amplifies the modeling complexity of ST data and compromises model interpretability. To this end, we propose a multi-factor ST prediction task that predicts partial ST data evolution under different factors, and combines them for a final prediction. We make two contributions to this task: an effective theoretical solution and a portable instantiation framework. Specifically, we first propose a theoretical solution called decomposed prediction strategy and prove its effectiveness from the perspective of information entropy theory. On top of that, we instantiate a novel model-agnostic framework, named spatio-temporal graph decomposition learning (STGDL), for multi-factor ST prediction. The framework consists of two main components: an automatic graph decomposition module that decomposes the original graph structure inherent in ST data into subgraphs corresponding to different factors, and a decomposed learning network that learns the partial ST data on each subgraph separately and integrates them for the final prediction. We conduct extensive experiments on four real-world ST datasets of two types of graphs, i.e., grid graph and network graph. Results show that our framework significantly reduces prediction errors of various ST models by 9.41% on average (35.36% at most). Furthermore, a case study reveals the interpretability potential of our framework.

==> 3-old-methodology.tex <==
\section{Methodology}\label{sec:method}

In this section, we elaborate on our proposed \model framework with the technical details (as shown in \figureautorefname~\ref{fig:framework}).

\subsection{Overview Framework}
% 从数据生成视角介绍模型设计原则

Classical data-driven methods model traffic flow data directly based on the global traffic graph $\mathcal{G}$ that mixes multiple traffic patterns. We innovatively propose a knowledge-guided traffic flow prediction framework \model, where the knowledge for traffic flow generation is derived from the laws of human mobility. As illustrated in \figureautorefname~\ref{fig:framework}, our \model consists of two parts: an implicit data generation process TPD and an explicit deep learning model HDN. In TPD, \ie Traffic Pattern Decomposition, we leverage the traffic flow generation knowledge to decompose the global traffic graph into multiple traffic patterns. Details of the implicit TPD will be given in Section~\ref{ssec:tpd}.

Over the implicit data generation process, we design a deep learning model, Hierarchical Decomposition Network (HDN), which stacks several subtractive residual learning blocks to disentangle each traffic pattern. In each block, we employ a graph attention-based spatio-temporal (ST) encoder to preserve the ST contextual information of traffic embeddings and introduce two decoders to decompose historical traffic observations and forecast future traffic status at the same time. Details are in Section~\ref{ssec:cdn}.

In our model, the knowledge of traffic flow data generation and the deep learning model are unified into the same framework, therefore our model can be easily trained in an end-to-end fashion.

\subsection{Traffic Pattern Decomposition}\label{ssec:tpd}
% 介绍图分解算法与理论证明

In this section, we propose a simple yet efficient traffic pattern decomposition scheme with two regularization terms preserving the pattern's property. Moreover, we provide a theoretical analysis for the proposed decomposition scheme.

\subsubsection{Decomposition with Regularization}

Given a global traffic graph $\mathcal{G}$, this module aims to decompose it into a set of sub-graphs $\left\{\tilde{\mathcal{G}}_1, \dots, \tilde{\mathcal{G}}_K\right\}$. Each of them denotes a kind of traffic pattern. Specifically, for the $k$-th traffic pattern $\tilde{\mathcal{G}}_k = \left(\tilde{\mathcal{V}}_k, \tilde{\mathcal{E}}_k, \tilde{\bm A}_k\right), 1\le k \le K$, we learn a mask matrix $\bm M_k$ to generate the corresponding adjacent matrix $\tilde{\bm A}_k$ as follows: 
\begin{equation}
    \tilde{\bm A}_k = \sigma\left(\bm M_k\right) \bm A,
\end{equation}
where $\sigma(\cdot)$ denotes the Sigmoid function that is used for constraining the edge weight ranging from $[0, 1]$. 

Directly using the decomposition results cannot ensure the traffic pattern's properties. For example, all patterns after decomposition are supposed to be able to reconstruct the input graph, \aka the pattern fidelity property. To this end, we introduce a fidelity regularization term $\mathcal{L}_f$ to minimize the reconstruction error as follows:
\begin{equation}\label{eq:rf}
    \mathcal{L}_f = D\left(\mathcal{G}, \mathcal{\hat G}\right),~~\mathrm{where}~~\mathcal{\hat G} = \bigcup_{k=1}^{K} \tilde{\mathcal{G}}
\end{equation}
In Eq.~\eqref{eq:rf}, $\mathcal{\hat G}$ is the estimation of the input global traffic graph, and $D(\cdot, \cdot)$ measures the distance or dissimilarity of two graphs. The classical graph similarity metric is graph edit distance. {\color{blue}However, the graph edit distance problem is NP-Hard\cite{zeng2009comparing}, and some relevant operators are not differentiable. For the sake of computational efficiency and ease of implementation, we propose a structural similarity method to compare the network structure between graphs, without considering the graph edit distance, using a previously developed measure for structural topological differences\cite{schieber2017quantification}. 

First, define the distance distribution $p$ of the graph, and $p\left(i,j\right)$ denotes the percentage of the number of nodes with distance $j$ from node $i$. The distance distribution contains much topological information of the graph, local information including the degree of nodes, closeness centrality, etc., and global information including diameter, average path length, number and size of connected blocks, etc.

The dissimilarity measure between traffic networks $\tilde{\mathcal{G}}_i$ and $\tilde{\mathcal{G}}_j$ with the number of nodes being N, is calculated by
\begin{equation}\label{eq:nnd}
    D\left(\tilde{\mathcal{G}}_i, \tilde{\mathcal{G}}_j\right)=w_1\sqrt{\frac{J(\mu_{\tilde{\mathcal{G}}_i},\mu_{\tilde{\mathcal{G}}_j})}{\log 2}} + w_2|\sqrt{NND(\tilde{\mathcal{G}}_i)}-\sqrt{NND(\tilde{\mathcal{G}}_j})|
\end{equation}

where TODO}

% 介绍一下D的计算

To avoid a trivial solution in which each pattern shares the same graph structure, we introduce another regularization term to ensure the pattern discrepancy property, \ie each traffic pattern is supposed to have more unique characteristics. The discrepancy regularization $\mathcal{L}_d$ is defined as:
\begin{equation}\label{eq:rd}
    \mathcal{L}_d = - \sum_{i=1}^{K-1} \sum_{j=i+1}^{K} D\left(\tilde{\mathcal{G}}_i, \tilde{\mathcal{G}}_j\right),~~1\le i, j \le K.
\end{equation}


% \subsubsection{Theoretical Analysis} ???@mouyu

\subsection{Hierarchical Decomposition Network}\label{ssec:cdn}
% 介绍分解网络的结构

In this section, we design a hierarchical decomposition network for multilevel learning of traffic patterns. The architecture design follows several key principles. Firstly, the architecture of our base block should be simple yet expressive. Secondly, the overall architecture should rely on the decomposed traffic patterns, \ie under the guidance of knowledge that how the citywide traffic flow data generate by human mobility of different traffic patterns. Finally, as a prerequisite to explore interpretability, the architecture should be extendable towards making its outputs human interpretable. Next, we discuss how these principles converge to the proposed hierarchical decomposition network.

\subsubsection{Spatio-Temporal Decomposition Block}

The proposed basic block, named as spatio-temporal decomposition (STD) block, serves at each level of the hierarchical decomposition network. As depicted in \figureautorefname~\ref{fig:block}, each STD block aims to preserve the ST contextual information over the corresponding traffic pattern by an ST encoder, so as to jointly decompose historical traffic observations and forecast future traffic status through two ST decoders. Here, we focus on describing the operation of $k$-th block in detail (note that the block index $k$ is dropped in \figureautorefname~\ref{fig:block} for brevity).

The $k$-th STD block accepts its respective input $\tilde{\mathcal{X}}^{(k)}$ and produces two outputs as follows:
\begin{equation}
    \hat{\mathcal{X}}^{(k)}, \hat{\bm{Y}}^{(k)} = \mathrm{STD}\left(\tilde{\mathcal{X}}^{(k)}\right),
\end{equation}
where $\hat{\mathcal{X}}^{(k)}$ denotes the historical traffic flow estimation of the decomposed traffic pattern, which provides constraints on the functional space so that the STD block can disentangle traffic flow of a certain pattern from the mixed citywide flow. $\hat{\bm{Y}}^{(k)}$ is the future traffic flow prediction of the relevant pattern. For the very first block in the model, its respective $\tilde{\mathcal{X}}^{(k)}$ is the overall model input $\mathcal{X}$, \ie 
\begin{equation}
    \tilde{\mathcal{X}}^{(0)}= \mathcal{X}.
\end{equation}
For the rest of the STD blocks, their inputs $\tilde{\mathcal{X}}^{(k)}$ are residual outputs of the previous blocks.

Within each STD block, there are two parts: ST encoder and ST decoder. Next, we introduce them in details.

\paratitle{ST Encoder}. ST encoder produces the traffic embedding of a certain pattern by integrating the temporal convolutional component with the graph attention mechanism. Specifically, for encoding the temporal traffic correlations, we adopt the 1-D causal convolution along the time dimension with a gated mechanism~\cite{yu2018spatio}. Given the traffic flow tensor $\tilde{\mathcal{X}}^{(k)} = \left(\tilde{\bm{X}}^{(k)}_{t-T+1}, \dots, \tilde{\bm{X}}^{(k)}_{t} \right)$ as the input, our temporal gated convolution (TGC) layer outputs a time-aware embedding for each spatial region:
\begin{equation}\label{eq:tgc}
    \left(\bm{H}^{(k)}_{t-T_{out}}, \dots, \bm{H}^{(k)}_{k,t}\right) = \mathrm{TGC}\left(\tilde{\bm{X}}^{(k)}_{t-T+1}, \dots, \tilde{\bm{X}}^{(k)}_{t} \right),
\end{equation}
where $\bm H^{(k)}_{t} \in \mathbb{R}^{N \times D}$ is the traffic embedding at the time step $t$ in the context of $k$-th traffic pattern $\tilde{\mathcal{G}}_k$. The $n$-th row $\bm{h}^{(k)}_{t,n} \in \mathbb{R}^{D}$ denotes the embedding of region $r_n$, where $D$ is the embedding dimension. $T_{out}$ is the length of the output embedding sequence. 

For capturing the spatial dependencies, we design our spatial graph attention (SGA) layer based on a graph attention-based message passing mechanism for time step $t$ as follows:
\begin{equation}
    \bm E^{(k)}_{t} = \mathrm{SGA}\left(\bm{H}^{(k)}_{t}, \tilde{\bm{A}}_{k}\right),
\end{equation}
where $\tilde{\bm{A}}_{k}$ is the adjacency matrix of the traffic pattern $\tilde{\mathcal{G}}_{k}$. After our SGA, we can obtain the refined embeddings $\left(\bm E^{(k)}_{t-T_{out}}, \dots, \bm E^{(k)}_{t}\right)$ by injecting the traffic pattern context. 

Our ST encoder is built with two ``sandwich'' structures, each of which represents as  $\mathrm{TGC}\to\mathrm{SGA}\to\mathrm{TGC}$. The output of the ST encoder is a traffic embedding tensor $\mathcal{H}^{(k)}$ that preserves the unique features of traffic pattern $\mathcal{G}_k$.

\paratitle{ST Decoder}. We design two ST decoders based on the embedding $\mathcal{H}^{(k)}$: one for disentanglement and another for prediction. The disentanglement decoder is implemented by two fully-connected (FC) layer as follows:
\begin{equation}
    \hat{\mathcal{X}}^{(k)} = \mathrm{FC_2}\left(\mathrm{FC}_1\left(\mathcal{H}^{(k)}\right)\right).
\end{equation}
$\mathrm{FC}_1$ is used along the time dimension, so as to align it with the input time window size. The second layer $\mathrm{FC}_2$ is applied for transforming the $D$-dimensional embedding into traffic flow that estimates the past flow observations of the $k$-th traffic pattern $\mathcal{G}_k$. 

The prediction decoder is composed of a temporal gated convolutional layer (Eq.~\eqref{eq:tgc}) followed by a fully-connected layer. The temporal convolutional layer takes the learned traffic embedding tensor $\mathcal{H}^{(k)}$ as input and outputs a singe-step prediction. Then, we produce the future traffic status relevant to the traffic pattern $\mathcal{G}_k$ through a fully-connected layer:
\begin{equation}
    \hat{\bm{Y}}^{(k)} = \mathrm{FC}_3\left(\mathrm{TGC}\left(\mathcal{H}^{(k)}\right)\right).
\end{equation}

In a word, we design our spatio-temporal decomposition block in a simple and expressive way. We employ the simple and widely-used 1-D convolution and attention mechanism to capture the temporal and spatial information of a specific traffic pattern. On the other hand, we adopt a ``sandwich'' structure and stack two sandwiches to improve the expression ability. 

\subsubsection{Hierarchical Decomposition Learning}

We devise a hierarchical decomposition learning scheme to inject the knowledge of human mobility data generation into the network structure, by hierarchically stacking several spatio-temporal decomposition blocks in a subtractive residual way.

Specifically, we subtract the well-estimated traffic flow of the $k$-th traffic pattern, $\hat{\mathcal{X}}^{(k)}$, from the mixed input flow of the $k$-th block, $\tilde{\mathcal{X}}^{(k)}$, which is described as follows:
\begin{equation}
    \tilde{\mathcal{X}}^{(k+1)} = \tilde{\mathcal{X}}^{(k)} - \hat{\mathcal{X}}^{(k)}.
\end{equation}
This subtractive residual connection removes the portion of traffic flow $\hat{\mathcal{X}}^{(k)}$ that it can approximate well, making the prediction task of the following traffic patterns belonging to the relevant blocks easier. After traffic flow of all patterns has been disentangled, the residual term should be zero. Therefore, we minimize the output of the last subtractive residual connection as follows:
\begin{equation}\label{eq:loss_r}
    \mathcal{L}_r = \tilde{\mathcal{X}}^{(K+1)},
\end{equation}
where $K$ is the total number of traffic patterns.

Then, we aggregate the partial prediction result $\hat{\bm{Y}}^{(k)}$ of each spatio-temporal decomposition block and obtain the final prediction as follows:
\begin{equation}
    \hat{\bm{Y}} = \sum_{k} \hat{\bm{Y}}^{(k)}.
\end{equation}
We treat each partial prediction $\hat{\bm{Y}}^{(k)}$ as the hierarchical decomposition of $\hat{\bm{Y}}$. Since $\hat{\bm{Y}}^{(k)}$ is responsible for the flow prediction of the $k$-th traffic pattern $\tilde{\mathcal{G}}_{k}$, we expect an accurate prediction of the citywide traffic flow $\hat{\bm{Y}}$ that mixes several traffic patterns. Because there are two different types of flows, we optimize the prediction task by minimizing the loss function below:
\begin{equation}\label{eq:loss_p}
    \mathcal{L}_p = \sum_{n=1}^{N} \lambda \left|y_{n,0} - \hat{y}_{n,0} \right| + (1-\lambda) \left|y_{n,1} - \hat{y}_{n,1} \right|,
\end{equation}
where $y_{n,0},y_{n,1}$ represent the ground truth of inflow and outflow respectively, and $\lambda$ is a parameter to balance the influence of each type of traffic flow.

More importantly, with the guidance of human mobility knowledge, the predicted flow of each block can have its own physical meaning in reality, such as the commuting flow and entertaining flow, which enhance the interpretability of the model's outputs. 

\subsection{Model Training}

In the learning process of our \model, we calculate the overall loss by incorporating the traffic pattern decomposition losses in Eq.~\eqref{eq:rf} and \eqref{eq:rd} and the hierarchical learning losses in Eq.~\eqref{eq:loss_r} and \eqref{eq:loss_p} into the joint learning objection:
\begin{equation}
    \mathcal{L}_{joint} = \mathcal{L}_f + \mathcal{L}_d + \mathcal{L}_r + \mathcal{L}_p.
\end{equation}

Our model can be trained end-to-end via the back-propagation algorithm. The entire training procedure can be summarized into Algo.~\ref{alg:train}.

{\color{red} An algorithm is needed.}


\subsection{Theoretical Analysis}

In this section, we conduct a theoretical analysis of \model to prove that our core decomposition scheme is theoretically guaranteed to be more effective in the traffic prediction problem.

\begin{theorem}
The graph decomposition scheme of our \model enables better traffic prediction performance.
\end{theorem}

\begin{proof}
The motivation behind the graph decomposition scheme is the divide-and-conquer strategy, where a complex problem is decomposed into different components each of which is tackled by an individual neural network. Following this idea, we prove the theorem by using three basic steps of the divide-and-conquer strategy: $i$) \textit{divide} the original problem into several subproblems, $ii$) \textit{conquer} each sub-problem by an individual neural network, and $iii$) \textit{combine} the solutions for the subproblems into a single solution.

Step $i$ divides the original traffic prediction problem into several smaller, independent subproblems. The traffic pattern of the original problem is exhibited as a complex graph where several patterns of human mobility mix together, so the original problem aims to forecast the \textit{mixed-pattern traffic flow}. On the contrary, step $i$ decomposes the mixed graph as several smaller subgraphs each of which represents a single pattern, resulting in a subproblem focusing on forecasting the \textit{single-pattern traffic flow}. To ensure the independence of these subproblems, we introduce a discrepancy regularization term in the traffic pattern decomposition, as shown in Eq.~\eqref{eq:rd}. 

To prove step $ii$, we introduce a lemma:
\begin{lemma}\label{lm:1}
The traffic prediction problem of a single pattern is simpler than that of a mixed pattern. 
\end{lemma}
This lemma implies that the subproblem is easier to handle than the original problem. In other words, we can solve each subproblem with a lower error rate even if we use a network with the same capacity as the original problem. Formally, if we use $d$ to denote the error rate of the original problem and $e_k, 1\le k \le K$ to denote the error rate of $k$-th subproblems, we can describe their relationship as follows:
\begin{equation}\label{eq:error_rate}
    \forall 1\le k \le K, e_k < d.
\end{equation}

% TODO: prove the third step.
% For simplicity and without loss of generality, we analyze the traffic flow of one node 用单个节点的方便后面lemma的证明
Step $iii$ combines the solutions for all subproblems into a single solution, and this solution is better than directly solving the original problem. Next, we give proof of it. For simplicity and without loss of generality, we focus on the traffic flow prediction of one spatial region. We use $y$ to denote the ground truth of the original problem, \ie the mixed-pattern traffic flow. For the $k$-th subproblem, we denote by $y_k$ the flow ground truth relevant to the $k$-th pattern, then we have $y = \sum_{k=1}^{K} y_k$.
% \begin{equation}
% y = \sum_{k=1}^{K} y_k.    
% \end{equation}
After combining solutions for the subproblems into a single solution by the divide-and-conquer strategy, we can calculate the overall error $e_s$ by
\begin{equation}
    e_s = \sum_{k=1}^{K} y_k * e_k.
\end{equation}
From Eq.~\eqref{eq:error_rate}, $e_k < d$ holds for $1\le k \le K$, so we have
\begin{equation}
e_s < \sum_{k=1}^{K} y_k * d < f*d.
\end{equation}
% \begin{equation}
% \begin{split}
%     e_s &< \sum_{k=1}^{K} y_k * d\\
%     &< f*d\\
% \end{split}
% \end{equation}
This means that the error of the combined solution is lower than that of directly solving the original problem. In other words, we can obtain better traffic prediction performance through the proposed graph decomposition scheme, which is principled by the divide-and-conquer strategy. 
\end{proof}

Here we provide the proof of Lemma~\ref{lm:1}.

\begin{proof}
    The proof of lemma 1.
\end{proof}


==> 3-old-theory.tex <==
% 解耦预测策略
% - 策略内容
%   - 交通数据生成过程
%   - 解耦预测策略
%   - 该策略的优势
% - 理论分析
%   - 策略优势的证明
%   - 交通流可预测性分析
%       - 可预测性性质
%       - 交通流可预测性

\section{Decomposed Prediction Strategy}\label{sec:theory}

This section first provides a theoretical solution, called decomposed prediction strategy, for the problem of multi-factor traffic prediction via a divide-and-conquer paradigm. Then, we prove the proposed solution's effectiveness.

\subsection{Strategy Details}

\paratitle{Traffic Data Generation Perspective.}
From the perspective of data generation, the process of traffic data generation can be affected by multiple factors~\cite{alessandretti2020scales}. 
% As shown in \fig~\ref{fig:data_gen}, 
Assuming there are $K$ factors, the traffic flow graph data $\mathcal{G}$ can be regarded as a mixture of all $\mathcal{G}_k = (G_k, \bm{X}_k), k\in[1, K]$. We use $\mathcal{G}_k$ to denote the traffic flow graph affected by the $k$-th factor. This effect involves two aspects: graph structure $G$ and traffic flow $\bm{X}$. Intuitively, we should decouple the graph structures corresponding to different factors, and then model the graph-based traffic flow under the influence of each factor separately. 

% TODO: 强调traffic flow random variable的概念

% In contrast, directly modeling the traffic data with a mixture of multiple factors will bring about the stacking of uncertainties from different factors, which reduces the predictability of traffic data. This will make the traffic prediction problem more difficult and thus degrade the model performance.

% 从数据生成的视角来看，交通数据的生成过程受到多种因素的影响~\cite{alessandretti2020scales}。如图xx所示，假设有K个影响因素，受第k种因素影响的交通数据为G_k，那么交通流图数据可以看作是所有G_k的混合。其中，每一个G_k包含两个方面：图结构和交通流。直觉上，我们应该解耦不同因素对应的图结构，然后分别建模每种因素影响下的交通流。因为混合多种因素会带来不同因素不确定性的叠加，这会提升交通预测问题的难度，从而降低模型表现。

\paratitle{Steps of Decomposed Prediction.}
There are three steps in our decomposed prediction strategy: 
% $i)$ \textit{Graph decomposition}. The graph structure $G$ containing a mixture of different factors is decomposed into several subgraph structures $\{G_k\}_{k=1}^{K}$ with constraints $\bigcup G_k = G$ and $\bigcap G_k = \emptyset$. The graph $G_k$ characterizes the $k$-th latent factor. $ii)$ \textit{Decomposed learning}. We learn the relevant traffic flow $\bm{X}_k$ over graph $G_k$ separately by the factor-specific ST encoder $f_k(\cdot)$. $iii)$ \textit{Prediction Integration}. We integrate the traffic prediction results corresponding to each factor and get the final traffic prediction via $\bm{X} = \sum_{k=1}^{K}\bm{X}_k$. 
\begin{itemize}[leftmargin=*]
    \item \textbf{Graph decomposition}. The traffic graph structure $G = (\mathcal{V}, \mathcal{E}, \bm{A})$ containing a mixture of different factors is decomposed into several traffic subgraphs $\{G_k\}_{k=1}^{K}$. The subgraph $G_k = (\mathcal{V}_k, \mathcal{E}_k, \bm{A}_k)$ characterizes the $k$-th latent factor. The decomposition process is constrained by $\bigcup \mathcal{E}_k = \mathcal{E}$ and $\bigcap \mathcal{E}_k = \emptyset$. 
    \item \textbf{Decomposed learning}. We learn the relevant traffic flow $\bm{X}_k$ over graph $G_k$ separately by the factor-specific ST encoder $f_k(\cdot)$. 
    \item \textbf{Prediction integration}. We integrate the traffic prediction results corresponding to each factor and get the final traffic prediction via $\bm{X} = \sum_{k=1}^{K}\bm{X}_k$.
\end{itemize}
Note that our proposed strategy is in the framework of the divide-and-conquer approach.
% 三步: 1.图分解, 2. 解耦学习, 3. 合并预测

\paratitle{Advantage of Decomposed Prediction Strategy.}
The proposed strategy can reduce the difficulty of the traffic prediction problem, and thus produce smaller errors. Specifically, directly modeling the traffic flow generated by multiple complex factors will bring about the stacking of uncertainties from different factors, which reduces the \textit{predictability of traffic flow}. This will make the traffic prediction problem more difficult and thus degrade the model performance. In contrast, inspired by the divide-and-conquer approach, the decomposed prediction strategy can characterize the influence of each latent factor separately. It makes the traffic flow data on the decomposed subgraph, \ie $\bm{X}_k$, easier to model than the data on the original graph, $\bm{X}$. In this way, we obtain an easier problem, namely multi-factor traffic prediction. The advantage of the proposed strategy is summarized in the following theorem.

\begin{theorem}\label{thm:stgy}
Assume the error lower bound of a traffic prediction problem is $E_o$. After introducing the decomposed prediction strategy and transforming the original problem into multi-factor traffic prediction, we can have an error lower bound $E_d$ with $E_d < E_o$.
\end{theorem}

In \thm~\ref{thm:stgy}, a smaller error lower bound means the difficulty of the corresponding problem is lower. A low-difficulty problem means it can be solved with smaller errors. The proof of \thm~\ref{thm:stgy} is provided in the following. 

\subsection{Theoretical Analysis}

\subsubsection{Proof of Strategy Advantage}

We here prove the advantage of our decomposed prediction strategy given in \thm~\ref{thm:stgy}. As shown in \tab~\ref{tab:analogy}, our strategy includes three steps related to parts of the divide-and-conquer approach. We translate these three parts into three lemmas and provide corresponding proofs. Then, we can prove \thm~\ref{thm:stgy} by using these three lemmas.

\begin{table}[t]
    \centering
    \caption{Analogy from decomposed prediction strategy to divide-and-conquer approach.}    \label{tab:analogy}
    \begin{tabular}{|rcl|}
    \hline 
    Graph decomposition & $\longrightarrow$ & Divide \\
    Decomposed learning  & $\longrightarrow$ & Conquer \\
    Prediction integration & $\longrightarrow$ & Combine \\
    \hline
    \end{tabular}
\end{table}

\begin{lemma}[Divide]\label{lem:divide}
    The graph decomposition step divides the original problem into a number of subproblems that are smaller instances of the same problem. 
\end{lemma}

\begin{IEEEproof}
Before delving into the proof, we give some necessary definitions.
\begin{mydef}[Problem Scale]\label{def:scale}
    Given a prediction problem $P$ on traffic flow graph $\mathcal{G}^{(t-T:t)} = (G, \bm{X}^{(t-T:t)})$ where $G = (\mathcal{V}, \mathcal{E}, \bm{A})$, we define the problem scale $B_P$ as the number of graph nodes, \ie $B_P = |\mathcal{V}|$.
\end{mydef}

\begin{mydef}[Problem Independence]
    Given two traffic prediction problems $P_1$ and $P_2$, the two problems are independent ($P_1 \perp P_2$) if and only if the graph edge sets $\mathcal{E}_1$ and $\mathcal{E}_2$ in the two problems are orthogonal, \ie $\mathcal{E}_1 \cap \mathcal{E}_2 = \emptyset$. 
\end{mydef}

According to the graph decomposition step, it decomposes the original traffic graph $G$ into $K$ traffic subgraphs, namely $\{G_k\}_{k=1}^{K}$. Consequently, the original traffic prediction problem $P$ defined on $G$ is divided into $K$ subproblems, namely $\{P_k\}_{k=1}^{K}$. Each subproblem aims to forecast the future traffic states $\bm{X}^{(t+1)}_k$ corresponding to $G_k$.

For any $P_k$, we know $G_k \subset G$ and their node numbers satisfy
\begin{equation}\label{eq:scale}
    \forall k \in [1, K], |\mathcal{V}_k| < |\mathcal{V}| \Rightarrow B_{P_k} < B_{P},
\end{equation}
Here $B_{P_k}$ is the scale of the $k$-th subproblem, while $B_P$ is the scale of the original problem. The derivation of \equ~\eqref{eq:scale} is based on Def.~\ref{def:scale}.

On the other hand, the traffic subgraphs satisfy $\bigcap \mathcal{E}_k = \emptyset$, so each pair of graph edge sets satisfy
\begin{equation}
    \forall j, k \in [1, K], \mathcal{E}_j \cap \mathcal{E}_k = \emptyset \Rightarrow P_j \perp P_k.
\end{equation}
This means that each two subproblems are independent.

\end{IEEEproof}

\begin{lemma}[Conquer]\label{lem:conquer}
    The decomposed learning step conquers the subproblems by solving them separately. The error lower bound of the $k$-th subproblem is $2e_k \sigma_k^2$. $e_k$ is the lower bound of error rate and $\sigma_k^2$ is the variance of the traffic flow random variable $X_k$ corresponding to the $k$-th subproblem.
\end{lemma}

\begin{IEEEproof}
According to \thm~\ref{thm:pred}, we know that the traffic flow predictability upper bound of the $k$-th subproblem ($\pi^{max}_k$) is greater than that of the original problem ($\pi^{max}$), \ie $\forall k \in[1, K], \pi^{max}_k > \pi^{max}$. 

Because predictability tells prediction accuracy~\cite{song2010limits}, the error rate lower bound of a traffic prediction problem can be denoted by $e = 1 - \pi^{max}$. For the $k$-th traffic prediction subproblem $P_k$, we have $e_k = 1 - \pi^{max}_k$ and it satisfies
\begin{equation}\label{eq:error_rate}
    \forall k \in [1, K], e_k < e,
\end{equation}
where $e$ is the error rate lower bound of directly solving the original traffic prediction problem $P$. 

% \begin{mydef}[Traffic Random Variable]
%     To emphasize the uncertainty and randomness of traffic flow data, we treat the traffic flow data $\bm{X}$ as samples of a traffic random variable $X$.
% \end{mydef}
% From the data generation perspective, traffic flow data is affected by multiple factors with uncertainties. 

From the data generation perspective, the traffic flow data of the $k$-th subproblem can be considered as samples of a random variable $X_k$. We use $\sigma^2_k$ to denote the variance of $X_k$. Then, we analyze the error lower bound of the $k$-th subproblem, namely $ELBO_k$. The error may come from two cases: $i)$ predictions are correct and $ii)$ predictions are incorrect. Thus, the error lower bound can be calculated by the expectation of errors in the two cases:
\begin{equation}\label{eq:elbo_k}
    ELBO_k = e_k \cdot r_k^{0} + (1-e_k) \cdot r_k^{1}. 
\end{equation}
where $e_k$ is the error rate lower bound of the $k$-th subproblem. $r_k^{0}$ is the error expectation when the predictions are incorrect, while $r_k^{1}$ is that when the predictions are correct. 

We know $r_k^{1} = 0$. As for $r_k^{0}$, it can be calculated by the error between each possible prediction and ground truth:
\begin{equation}\label{eq:err_exp}
    r_k^{0} = \sum_i p_i^{(k)} \sum_j p_j^{(k)} \left(x_j^{(k)} - x_i^{(k)}\right)^2,
\end{equation}
where $x_i^{(k)}$ is a ground truth with possibility $p_i^{(k)}$, and $x_j^{(k)}$ is a prediction with possibility $p_j^{(k)}$. Solving \equ~\eqref{eq:err_exp} is equivalent to finding the solution of $\mathbb{E}[(X-Y)^2]$ with constraint $X \perp Y$. By derivations in Appx.~\ref{xx}, we know that the solution is $r_k^{0} = 2\sigma_k^2$. Taking $r_k^{1}$ and $r_k^{0}$ into \equ~\eqref{eq:elbo_k}, we can have
\begin{equation}\label{eq:elbo_k_ana}
    ELBO_k = e_k \cdot 2\sigma_k^2 + (1-e_k) \cdot 0 =  2 e_k \sigma_k^2.
\end{equation}
That is, the error lower
bound of the $k$-th subproblem is $2 e_k \sigma_k^2$.
\end{IEEEproof}

\begin{lemma}[Combine]\label{lem:combine}
    The prediction integration step combines the solutions to the subproblems into the solution for the original problem. The error lower bound of the combined solution is $\sum_{k=1}^{K} 2 e_k \sigma_k^2$. 
    % smaller than that of the direct solution not using the decomposed prediction strategy.
\end{lemma}

\begin{IEEEproof}
By combing the solutions to the subproblems, we can have a combined solution for the original problem. From Lemma~\ref{lem:divide}, the subproblems are independent of each other. This means that the covariance of any two subproblems is zero, thereby making the covariance of the relevant traffic random variables zero. Therefore, the error lower bound of the combined solution ($E_d$) can be calculated by the summation of the lower bounds of all subproblems:
\begin{equation}\label{eq:elbo_dac}
    E_d = \sum_{k=1}^{K} ELBO_k = \sum_{k=1}^{K} 2 e_k \sigma_k^2.
\end{equation}
The proof of Lemma~\ref{lem:combine} is finished. 

% Similar to \equ~\eqref{eq:elbo_k_ana}, we can derive the error lower bound of the original problem as
% \begin{equation}\label{eq:elbo_org}
% E_o = 2 e \sigma^2, \st \sigma^2 = \sum_{k=1}^{K} \sigma_k^2
% \end{equation}
% where $e$ is the error rate lower bound of directly solving the original traffic prediction problem. $\sigma^2$ is the variance of the traffic random variable $X$ corresponding to the original problem $P$. The constraint $\sigma^2 = \sum_{k=1}^{K} \sigma_k^2$ is derived from Lemma~\ref{lem:divide}. Because the original problem is divided into $K$ \textit{independent} subproblems, the covariance of any two subproblems is zero. This indicates variances of all $X_k$ sums up to the variance of $X$.

% Comparing \equ~\eqref{eq:elbo_dac} and \equ~\eqref{eq:elbo_org} with the help of \equ~\eqref{eq:error_rate}, we have
% \begin{equation}
%     E_d = \sum_{k=1}^{K} 2 e_k \sigma_k^2 < \sum_{k=1}^{K} 2 e \sigma_k^2 = 2 e \sigma^2 = E_o.
% \end{equation}
% This equation shows that the error lower bound of the combined solution is smaller than that of the direct solution not using the decomposed prediction strategy.


% Comparing \equ~\eqref{eq:elbo} to \eqref{eq:elbo_k_ana} with the help of \equ~\eqref{eq:error_rate}, we have 
% \begin{equation}
%     ELBO_k = 2 e_k \sigma_k^2 < 2 e \sigma^2 = ELBO.
% \end{equation}
% Therefore, the error lower bound of each subproblem is small than that of the original problem. That is, each subproblem is easier than the original problem.
\end{IEEEproof}

Next, we give the proof of \thm~\ref{thm:stgy} by combing the conclusions of Lemma~\ref{lem:divide}, Lemma~\ref{lem:conquer}, and Lemma~\ref{lem:combine}.
\begin{IEEEproof}
Assume the error lower bound of a traffic prediction problem is $E_o$. From Lemma~\ref{lem:conquer}, we know that $E_o$ is proportional to the error rate lower bound and the variance of the corresponding traffic random variable. Similar to \equ~\eqref{eq:elbo_k_ana}, we can derive the error lower bound of the original problem as
\begin{equation}\label{eq:elbo_org}
E_o = 2 e \sigma^2, \st \sigma^2 = \sum_{k=1}^{K} \sigma_k^2
\end{equation}
where $e$ is the error rate lower bound of directly solving the original traffic prediction problem. $\sigma^2$ is the variance of the traffic random variable $X$ corresponding to the original problem $P$. The constraint $\sigma^2 = \sum_{k=1}^{K} \sigma_k^2$ is derived from Lemma~\ref{lem:divide}. Because the original problem is divided into $K$ \textit{independent} subproblems, the covariance of any two subproblems is zero. This indicates variances of all traffic random variables $X_k$ sum up to the variance of $X$.

Comparing \equ~\eqref{eq:elbo_dac} and \equ~\eqref{eq:elbo_org} with the help of \equ~\eqref{eq:error_rate}, we have
\begin{equation}
    E_d = \sum_{k=1}^{K} 2 e_k \sigma_k^2 < \sum_{k=1}^{K} 2 e \sigma_k^2 = 2 e \sigma^2 = E_o.
\end{equation}
% This equation shows that the error lower bound of the combined solution is smaller than that of the direct solution not using the decomposed prediction strategy.
This means that after introducing the decomposed prediction strategy, we can have a smaller error lower bound compared with directly solving the original problem.

% After introducing the decomposed prediction strategy and transforming the original problem into multi-factor traffic prediction, we can have an error lower bound $E_d$ with $E_d < E_o$.

% There are three steps in the decomposed prediction strategy, and they are designed according to the divide-and-conquer approach. Thus, we look into them in a  to xx the decomposed prediction strategy as three 

\end{IEEEproof} 

\subsubsection{Analysis of Traffic Flow Predictability}\label{ssec:predictability}

Traffic flow predictability describes the extent to which urban traffic flow is predictable with only past traffic flow observations. 
The traffic flow data of a node is naturally a time series of discrete values. This allows us to use tools from information theory, including entropy~\cite{brabazon2008natural} and Fano's inequality~\cite{cover2006elements}, to measure the predictability of traffic flow. 

% Our approach is inspired by xx, is inspired by the seminal work of Song et al. who incorporate information theory into time series analysis to measure the limited predictability of individual mobility [29]. Differently, we estimate the traffic dynamics patterns at the population level, rather than at the individual level.

% The generation of traffic flow series can be viewed as a stochastic process, where the traffic flow volume transit among different states. Taking xx as an example, xx.

Since entropy is the most fundamental quantity capturing the degree of predictability characterizing a time series~\cite{Brabazon2008}, we exploit it to quantify the uncertainty of node traffic flow and the degree of predictability. The results of a whole traffic flow graph can then be quantified by that of all nodes of it.  

% 交通流的熵定义。
\paratitle{Traffic Flow Entropy.}
From the perspective of data generation, the traffic flow may include the influence of multiple factors. Assume there are $K$ factors in total. We use $X_k$ ($k \in [1, K]$) to denote the traffic flow random variable relevant to the $k$-th factor, and its entropy $S_k$ is defined as
\begin{equation}\label{eq:sf_ent}
    S_k = H(X_k) = -\sum_{i} p(x_i) \log p(x_i),
\end{equation}
where $H(X_k)$ is the information entropy of random variable $X_k$, and $p(x_i)$ is the probability of event $X_k = x_i$. 

The complete traffic flow distribution is the joint distribution of all traffic random variables, namely $\{X_k\}_{k=1}^{K}$.
According to the definition of joint entropy, the entropy of the complete traffic flow distribution can be defined as  
\begin{equation}\label{eq:mf_ent}
    S = H(X_1, X_2, \dots, X_K) = \sum_{k=1}^{K} H(X_k|X_{k-1}, \dots, X_1),
\end{equation}
where $H(X_k|X_{k-1}, \dots, X_1)$ is the conditional entropy. Based on the traffic flow entropy in \equ~\eqref{eq:sf_ent} and \equ~\eqref{eq:mf_ent}, we can have the following lemma. 

% lemma：熵的关系
\begin{lemma}\label{lem:ent}
    The traffic flow entropy of any single factor ($S_k$) is smaller than that of multiple factors ($S$), \ie $\forall k\in[1, K], S_k < S$. 
\end{lemma}

\begin{IEEEproof}
    There are two steps to prove this lemma: $i)$ proving $S_1 < S$. $ii)$ extending the conclusion of $S_1$ to $S_k$.

    Firstly, we expand the summation term in \equ~\eqref{eq:mf_ent}:
    \begin{equation}\label{eq:ent_ss1}
    \begin{split}
        S &=H(X_1, X_2, \dots, X_K)\\
        &= H(X_1) + H(X_2| X_1) + \dots + H(X_K|X_{K-1},\dots,X_1)\\
        &\ge H(X_1) = S_1.\\
    \end{split}
    \end{equation}
    The last step is derived from the non-negativity of conditional entropy. It means that in the second step, each term after $H(X_1)$, such as $H(X_2|X_1)$, is non-negative. 

    Secondly, according to the symmetry of entropy, entropy should be unchanged if the outcomes $X_k$ are re-ordered. Therefore, we can rewrite the expression of $S$ as
    \begin{equation}
       S = (X_k, X_1, \dots, X_{k-1}, X_{k+1}, \dots, X_K).
    \end{equation}
    Here, we adjust $X_k$ from the $k$-th position to the first position. This operation does not change the value of entropy. By using the rules of \equ~\eqref{eq:ent_ss1}, we can obtain
    \begin{equation}
        S_k \le S, k \in [1, K].
    \end{equation}
    The equal sign is obtained when the traffic flow of all factors is the same. This is nearly impossible in real-world scenarios, so we remove the equal sign and reach the final conclusion that $\forall k \in [1, K], S_k < S$.
\end{IEEEproof}

% 交通流熵与可预测性的关系
\paratitle{Traffic Flow Predictability.}
The entropy of node traffic flow allows us to measure the predictability $\pi$ that a suitable
predictive algorithm can correctly predict the future traffic flow state. According to Ref.~\cite{song2010limits}, the predictability measure is subject to Fano’s inequality. Specifically, if the traffic flow volume is updated in $M$ states with the time, then its predictability $\pi \le \pi^{max}$. The upper bound of predictability, namely $\pi^{max}$, can be calculated by solving
\begin{equation}\label{eq:pi_max}
    S = H(\pi^{max}) + (1-\pi^{max}) \log(M-1).
\end{equation}
Here, $H(\pi^{max})$ is the entropy of $\pi^{max}$ and can be derived by $H(\pi^{max}) = -\pi^{max}\log(\pi^{max})-(1-\pi^{max})\log(1-\pi^{max})$. For a graph node with $\pi^{max} = 0.6$, we can predict its traffic flow state accurately only in $60\%$ of the cases. That is, $60\%$ is the upper bound of probability for any algorithms attempting to predict the node traffic flow state. 

Similar to traffic entropy, we can define the predictability upper bound of any single factor, namely $\pi_k^{max}$. Then, we have the following theorem.

% 定理2：可预测性的关系
\begin{theorem}\label{thm:pred}
    For traffic flow data, the predictability upper bound of any single factor ($\pi_k^{max}$) is greater than that of multiple factors ($\pi^{max}$), \ie $\forall k\in[1, K], \pi_k^{max} > \pi^{max}$. 
\end{theorem}

This indicates that if we divide the original traffic prediction problem into several smaller subproblems relevant to single factors, we can obtain subproblems with greater predictability compared with the original one. Next, we give the proof of \thm~\ref{thm:pred}

\begin{IEEEproof}
Taking $H(\pi^{max})$ into \equ~\eqref{eq:pi_max}, we can obtain the relation of entropy and predictability as follows:
\begin{equation}\label{eq:ent_pred}
\begin{split}
    S = &-\pi^{max}\log(\pi^{max})-(1-\pi^{max})\log(1-\pi^{max})\\
    &+ (1-\pi^{max}) \log(M-1)\\
\end{split}
\end{equation}
Once the traffic flow data is given, the state number $M$ will be fixed and can be treated as a constant. This makes the entropy $S$ a function of $\pi^{max}$, \ie $S(\pi^{max})$. Next, we analyze the properties of this function.

Taking the first-order derivation of $S$ over $\pi^{max}$ yields
\begin{equation}\label{eq:first_order}
     S' = -\log(\pi^{max}) + \log(1-\pi^{max}) - \log(M-1).
\end{equation}
Then, taking the second-order derivation of $S$ yields
\begin{equation}
    S'' = \frac{1}{\pi^{max}(1-\pi^{max})}.
\end{equation}
Since $\pi^{max} \in [0, 1]$, the inequality $S'' < 0$ always holds. This indicates that $S$ is a concave function on $\pi^{max}$ and $S$ has a maximum value. 

Let the first-order derivative in \equ~\eqref{eq:first_order} be zero to obtain the maximum value point as $\pi^{max} = 1/M$. When $\pi^{max} > 1/M$, $S$ is a monotonically decreasing function of $\pi^{max}$. Oppositely, when $\pi^{max} < 1/M$, $S$ is a monotonically increasing function of $\pi^{max}$. 

Since it was found that $\pi^{max} > 1/M$ usually holds for human mobility~\cite{song2010limits, wang2015predictability}, $S$ can generally be considered as a monotonically decreasing function of $\pi^{max}$. This means that the larger $S$ is, the smaller the corresponding $\pi^{max}$ is. According to Lemma~\ref{lem:ent}, $S_k$ is smaller than $S$. Therefore, $\pi_k^{max}$ is greater than $\pi^{max}$, \ie $\forall k \in [1, K], \pi_k^{max} > \pi^{max}$.
\end{IEEEproof}


